Further Results on an Abstract Model for Branching and its Application to Mixed-Integer Programming

A key ingredient in branch and bound (B&B) solvers for mixed-integer programming (MIP) is the selection of branching variables since poor or arbitrary selection can affect the size of the resulting search trees by orders of magnitude. A recent article by Le Bodic and Nemhauser [Mathematical Programming, (2017)] investigated variable selection rules by developing a theoretical model of B&B trees from which they developed some new, effective scoring functions for MIP solvers. In their work, Le Bodic and Nemhauser left several open theoretical problems, solutions to which could guide the future design of variable selection rules. In this article, we first solve many of these open theoretical problems. We then implement an improved version of the model-based branching rules in SCIP 6.0, a state-of-the-art academic MIP solver, in which we observe an 11% geometric average time and node reduction on instances of the MIPLIB 2017 Benchmark Set that require large B&B trees.

==> rubberband_all.tex <==
  30n20b8 &\textbf{3} & 281.40 & 138.00 & \textbf{+0} & 0.92 & 1.26 & \textbf{+0} & \textbf{0.70} & \textbf{0.56} \\
  CMS750\_4 &\textbf{3} & \textbf{857.93} & \textbf{11.91k} & \textbf{+0} & 1.25 & 1.03 & \textbf{+0} & 2.15 & 2.06 \\
  air05 &\textbf{3} & \textbf{30.10} & \textbf{333.67} & \textbf{+0} & 1.20 & 1.91 & \textbf{+0} & 1.17 & 1.19 \\
  app1-1 &\textbf{3} & 5.97 & \textbf{4.00} & \textbf{+0} & 1.01 & \textbf{1.00} & \textbf{+0} & \textbf{0.99} & \textbf{1.00} \\
  app1-2 &\textbf{3} & 1.04k & 68.33 & \textbf{+0} & \textbf{0.83} & \textbf{0.62} & \textbf{+0} & 1.28 & 0.85 \\
  assign1-5-8 &\textbf{3} & 3.35k & 5.94m & \textbf{+0} & 0.96 & 0.93 & \textbf{+0} & \textbf{0.85} & \textbf{0.83} \\
  beasleyC3 &\textbf{3} & 22.57 & \textbf{2.00} & \textbf{+0} & 1.00 & \textbf{1.00} & \textbf{+0} & \textbf{1.00} & \textbf{1.00} \\
  binkar10\_1 &\textbf{3} & 28.47 & 2.58k & \textbf{+0} & \textbf{0.79} & 0.88 & \textbf{+0} & 0.83 & \textbf{0.86} \\
  bnatt400 &\textbf{3} & 1.18k & \textbf{6.85k} & \textbf{+0} & 0.96 & 1.07 & \textbf{+0} & \textbf{0.96} & 1.07 \\
  bnatt500 &\textbf{3} & 5.02k & 30.07k & \textbf{+0} & 0.97 & \textbf{0.96} & \textbf{+0} & \textbf{0.97} & \textbf{0.96} \\
  bppc4-08 &0 & - & - & \textbf{+2} & - & - & \textbf{+2} & - & - \\
  brazil3 &\textbf{3} & 4.01k & \textbf{1.69k} & \textbf{+0} & \textbf{1.00} & 1.47 & \textbf{+0} & 1.04 & 1.39 \\
  chromaticindex512-7 &\textbf{3} & \textbf{2.21k} & \textbf{5.89k} & \textbf{+0} & 1.01 & 1.24 & \textbf{+0} & 1.01 & 1.24 \\
  co-100 &\textbf{2} & 4.53k & \textbf{6.11k} & \textbf{+0} & \textbf{0.93} & 1.64 & \textbf{+0} & 1.09 & 2.01 \\
  cod105 &\textbf{3} & \textbf{315.37} & \textbf{105.00} & \textbf{+0} & 1.16 & 2.05 & \textbf{+0} & 1.18 & 2.04 \\
  cost266-UUE &\textbf{3} & 3.18k & 234.69k & \textbf{+0} & 1.34 & 1.46 & \textbf{+0} & \textbf{0.96} & \textbf{0.95} \\
  csched007 &\textbf{3} & 3.11k & 266.24k & \textbf{+0} & \textbf{0.53} & \textbf{0.51} & \textbf{+0} & 0.71 & 0.57 \\
  csched008 &\textbf{3} & \textbf{1.03k} & \textbf{94.19k} & \textbf{+0} & 1.27 & 1.24 & \textbf{+0} & 1.36 & 1.42 \\
  dano3\_3 &\textbf{3} & \textbf{106.70} & \textbf{12.33} & \textbf{+0} & 1.10 & 1.68 & \textbf{+0} & 1.02 & 1.41 \\
  dano3\_5 &\textbf{3} & 307.80 & 165.00 & \textbf{+0} & \textbf{0.86} & \textbf{0.89} & \textbf{+0} & 0.89 & 1.04 \\
  drayage-100-23 &\textbf{3} & 16.83 & 33.33 & \textbf{+0} & 0.95 & 1.03 & \textbf{+0} & \textbf{0.89} & \textbf{0.90} \\
  drayage-25-23 &\textbf{3} & 1.29k & \textbf{106.45k} & -2 & 4.99 & 18.14 & -2 & \textbf{0.97} & 2.67 \\
  eil33-2 &\textbf{3} & 70.93 & 797.00 & \textbf{+0} & \textbf{0.89} & \textbf{0.91} & \textbf{+0} & 0.97 & 0.97 \\
  fast0507 &\textbf{3} & \textbf{217.13} & \textbf{840.00} & \textbf{+0} & 1.44 & 1.54 & \textbf{+0} & 1.20 & 1.15 \\
  fastxgemm-n2r6s0t2 &\textbf{3} & 605.93 & 113.70k & \textbf{+0} & 1.35 & 1.42 & \textbf{+0} & \textbf{0.76} & \textbf{0.73} \\
  fiball &1 & 1.47k & 3.56k & \textbf{+1} & \textbf{0.89} & \textbf{0.80} & \textbf{+1} & 1.17 & 1.16 \\
  gen-ip002 &\textbf{3} & 1.55k & 5.59m & \textbf{+0} & \textbf{0.91} & \textbf{0.93} & \textbf{+0} & 0.96 & 1.00 \\
  gen-ip054 &\textbf{3} & 3.04k & 12.77m & \textbf{+0} & \textbf{0.63} & \textbf{0.62} & \textbf{+0} & 0.63 & 0.63 \\
  glass-sc &\textbf{3} & 3.16k & 278.80k & \textbf{+0} & \textbf{0.93} & \textbf{0.96} & \textbf{+0} & 0.95 & 0.98 \\
  glass4 &\textbf{3} & \textbf{2.17k} & \textbf{1.73m} & \textbf{+0} & 1.54 & 2.37 & \textbf{+0} & 1.14 & 1.63 \\
  graph20-20-1rand &2 & 5.17k & 38.68k & +0 & \textbf{0.34} & \textbf{0.37} & \textbf{+1} & 0.49 & 0.49 \\
  graphdraw-domain &\textbf{3} & \textbf{1.39k} & \textbf{2.52m} & \textbf{+0} & 1.15 & 1.11 & \textbf{+0} & 1.03 & 1.01 \\
  h80x6320d &\textbf{3} & \textbf{105.67} & \textbf{4.00} & \textbf{+0} & 1.00 & \textbf{1.00} & \textbf{+0} & 1.00 & \textbf{1.00} \\
  icir97\_tension &0 & - & - & \textbf{+3} & - & - & +1 & - & - \\
  irp &\textbf{3} & \textbf{12.90} & \textbf{5.33} & \textbf{+0} & 1.01 & \textbf{1.00} & \textbf{+0} & 1.00 & \textbf{1.00} \\
  istanbul-no-cutoff &\textbf{3} & 179.57 & 302.33 & \textbf{+0} & \textbf{0.95} & 1.03 & \textbf{+0} & 1.02 & \textbf{0.99} \\
  map10 &\textbf{3} & \textbf{775.90} & \textbf{1.15k} & \textbf{+0} & 1.01 & 1.32 & \textbf{+0} & 1.11 & 1.43 \\
  map16715-04 &\textbf{3} & \textbf{1.75k} & \textbf{1.73k} & \textbf{+0} & 1.17 & 1.35 & \textbf{+0} & 1.21 & 1.31 \\
  markshare\_4\_0 &\textbf{3} & 320.37 & 2.51m & \textbf{+0} & \textbf{0.78} & \textbf{0.79} & \textbf{+0} & 0.87 & 0.88 \\
  mas74 &\textbf{3} & 2.29k & 7.07m & \textbf{+0} & 0.89 & 0.84 & \textbf{+0} & \textbf{0.77} & \textbf{0.78} \\
  mas76 &\textbf{3} & 132.87 & 301.16k & \textbf{+0} & 0.98 & 1.02 & \textbf{+0} & \textbf{0.90} & \textbf{0.88} \\
  mc11 &\textbf{3} & \textbf{112.33} & 2.26k & \textbf{+0} & 1.01 & \textbf{0.95} & \textbf{+0} & 1.55 & 2.12 \\
  mcsched &\textbf{3} & 240.10 & \textbf{11.39k} & \textbf{+0} & \textbf{0.99} & 1.31 & \textbf{+0} & 1.00 & 1.08 \\
  mik-250-20-75-4 &\textbf{3} & 37.23 & 16.05k & \textbf{+0} & \textbf{0.74} & \textbf{0.73} & \textbf{+0} & 0.79 & 0.76 \\
  mzzv11 &\textbf{3} & 336.90 & 1.57k & \textbf{+0} & \textbf{0.90} & 0.98 & \textbf{+0} & 0.94 & \textbf{0.80} \\
  mzzv42z &\textbf{3} & \textbf{168.13} & \textbf{259.67} & \textbf{+0} & 1.26 & 1.22 & \textbf{+0} & 1.19 & 1.34 \\
  n2seq36q &\textbf{3} & 921.67 & 4.12k & \textbf{+0} & \textbf{0.94} & \textbf{0.52} & \textbf{+0} & 0.95 & 0.86 \\
  n5-3 &\textbf{3} & \textbf{30.50} & \textbf{785.33} & \textbf{+0} & 1.07 & 1.17 & \textbf{+0} & 1.06 & 1.22 \\
  neos-1445765 &\textbf{3} & \textbf{59.53} & \textbf{72.33} & \textbf{+0} & 1.03 & 1.29 & \textbf{+0} & 1.01 & \textbf{1.00} \\
  neos-1456979 &\textbf{1} & - & - & -1 & - & - & -1 & - & - \\
  neos-1582420 &\textbf{3} & 37.30 & \textbf{664.33} & \textbf{+0} & \textbf{0.99} & 1.02 & \textbf{+0} & 1.21 & 1.67 \\
  neos-2657525-crna &0 & - & - & +0 & - & - & \textbf{+1} & - & - \\
  neos-3004026-krka &\textbf{3} & 68.13 & 5.25k & \textbf{+0} & \textbf{0.82} & \textbf{0.66} & \textbf{+0} & 0.82 & \textbf{0.66} \\
  neos-3024952-loue &2 & 1.22k & 135.87k & \textbf{+1} & 1.25 & 0.92 & \textbf{+1} & \textbf{0.99} & \textbf{0.74} \\
  neos-3083819-nubu &\textbf{3} & 14.93 & 2.33k & \textbf{+0} & \textbf{0.86} & 1.01 & \textbf{+0} & 0.89 & \textbf{1.00} \\
  neos-3216931-puriri &\textbf{1} & - & - & -1 & - & - & -1 & - & - \\
  neos-3402294-bobin &\textbf{3} & 1.84k & 12.76k & \textbf{+0} & 1.02 & 1.44 & \textbf{+0} & \textbf{0.68} & \textbf{0.53} \\
  neos-3627168-kasai &0 & - & - & \textbf{+1} & - & - & \textbf{+1} & - & - \\
  neos-4413714-turia &\textbf{3} & 387.20 & \textbf{2.00} & \textbf{+0} & \textbf{0.99} & \textbf{1.00} & \textbf{+0} & 1.00 & \textbf{1.00} \\
  neos-4722843-widden &\textbf{3} & \textbf{1.60k} & \textbf{2.62k} & \textbf{+0} & 1.12 & 1.15 & \textbf{+0} & 1.01 & 1.01 \\
  neos-4738912-atrato &\textbf{3} & 1.02k & 103.05k & \textbf{+0} & \textbf{0.71} & \textbf{0.60} & \textbf{+0} & 0.87 & 0.82 \\
  neos-5107597-kakapo &\textbf{3} & \textbf{2.10k} & \textbf{682.60k} & -2 & 2.67 & 3.52 & -1 & 1.85 & 2.23 \\
  neos-5188808-nattai &\textbf{3} & 2.22k & 27.40k & \textbf{+0} & \textbf{0.83} & \textbf{0.69} & \textbf{+0} & 0.84 & 0.81 \\
  neos-5195221-niemur &\textbf{3} & \textbf{2.68k} & \textbf{21.97k} & \textbf{+0} & 1.10 & 1.09 & \textbf{+0} & 1.25 & 1.31 \\
  neos-848589 &\textbf{1} & - & - & \textbf{+0} & - & - & -1 & - & - \\
  neos-860300 &\textbf{3} & \textbf{16.73} & \textbf{2.00} & \textbf{+0} & \textbf{1.00} & \textbf{1.00} & \textbf{+0} & 1.01 & \textbf{1.00} \\
  neos-911970 &\textbf{2} & \textbf{1.12k} & \textbf{623.61k} & -1 & 2.55 & 2.37 & -1 & 2.32 & 1.27 \\
  neos-933966 &\textbf{3} & 1.87k & 582.00 & \textbf{+0} & 1.60 & \textbf{0.91} & \textbf{+0} & \textbf{0.93} & 1.03 \\
  neos-950242 &\textbf{3} & 283.60 & 71.33 & \textbf{+0} & \textbf{0.82} & \textbf{0.72} & \textbf{+0} & 0.85 & 0.74 \\
  neos-960392 &\textbf{3} & \textbf{1.22k} & \textbf{65.67} & \textbf{+0} & 1.09 & 1.04 & \textbf{+0} & 1.09 & 1.04 \\
  neos17 &\textbf{3} & 22.07 & \textbf{16.59k} & \textbf{+0} & 1.17 & 1.06 & \textbf{+0} & \textbf{1.00} & 1.03 \\
  neos5 &\textbf{3} & 104.37 & 255.57k & \textbf{+0} & \textbf{0.92} & \textbf{0.96} & \textbf{+0} & 1.12 & 1.19 \\
  net12 &\textbf{3} & 1.34k & 2.07k & \textbf{+0} & \textbf{0.71} & \textbf{0.85} & \textbf{+0} & 0.73 & 0.88 \\
  netdiversion &\textbf{3} & \textbf{951.75} & \textbf{13.00} & -1 & 1.66 & 2.08 & \textbf{+0} & 2.30 & 3.96 \\
  nexp-150-20-8-5 &\textbf{2} & 2.35k & \textbf{3.60k} & \textbf{+0} & 1.34 & 2.18 & \textbf{+0} & \textbf{0.92} & 2.09 \\
  ns1208400 &\textbf{3} & 513.60 & \textbf{1.26k} & \textbf{+0} & 0.79 & 1.21 & \textbf{+0} & \textbf{0.79} & 1.21 \\
  ns1644855 &\textbf{2} & 2.09k & \textbf{8.00} & -1 & 1.01 & \textbf{1.00} & -1 & \textbf{0.99} & \textbf{1.00} \\
  ns1830653 &\textbf{3} & \textbf{115.40} & 6.23k & \textbf{+0} & 1.24 & 1.20 & \textbf{+0} & 1.23 & \textbf{0.93} \\
  ns1952667 &\textbf{3} & 1.56k & \textbf{3.19k} & \textbf{+0} & \textbf{0.53} & 1.16 & \textbf{+0} & 0.53 & 1.16 \\
  nu25-pr12 &\textbf{3} & 6.60 & 97.00 & \textbf{+0} & \textbf{0.99} & \textbf{0.88} & \textbf{+0} & 1.04 & 0.97 \\
  nursesched-sprint02 &\textbf{3} & \textbf{39.87} & 13.00 & \textbf{+0} & 1.02 & \textbf{0.97} & \textbf{+0} & 1.01 & \textbf{0.97} \\
  nw04 &\textbf{3} & \textbf{23.87} & \textbf{7.33} & \textbf{+0} & 1.01 & \textbf{1.00} & \textbf{+0} & 1.00 & \textbf{1.00} \\
  p200x1188c &\textbf{3} & 2.90 & \textbf{3.00} & \textbf{+0} & \textbf{0.99} & \textbf{1.00} & \textbf{+0} & \textbf{0.99} & \textbf{1.00} \\
  peg-solitaire-a3 &\textbf{1} & \textbf{4.09k} & \textbf{1.92k} & \textbf{+0} & 1.53 & 2.02 & \textbf{+0} & 1.52 & 2.02 \\
  pg &\textbf{3} & 20.47 & 552.67 & \textbf{+0} & \textbf{0.99} & 0.94 & \textbf{+0} & 0.99 & \textbf{0.92} \\
  pg5\_34 &\textbf{3} & 2.09k & 191.13k & \textbf{+0} & 0.84 & 0.98 & \textbf{+0} & \textbf{0.72} & \textbf{0.90} \\
  physiciansched6-2 &\textbf{1} & \textbf{165.20} & \textbf{151.00} & \textbf{+0} & 2.15 & 12.62 & \textbf{+0} & 1.52 & 7.28 \\
  piperout-08 &\textbf{3} & 858.30 & 604.00 & \textbf{+0} & \textbf{0.93} & 0.81 & \textbf{+0} & 1.05 & \textbf{0.62} \\
  piperout-27 &\textbf{3} & \textbf{320.93} & \textbf{174.00} & \textbf{+0} & 1.65 & 2.13 & \textbf{+0} & 1.49 & 1.17 \\
  pk1 &\textbf{3} & 149.93 & 386.87k & \textbf{+0} & 1.03 & 1.06 & \textbf{+0} & \textbf{0.96} & \textbf{0.96} \\
  qap10 &\textbf{3} & 108.17 & \textbf{3.33} & \textbf{+0} & \textbf{0.99} & \textbf{1.00} & \textbf{+0} & 1.03 & \textbf{1.00} \\
  rail507 &\textbf{3} & 255.57 & 1.32k & \textbf{+0} & 1.03 & 0.80 & \textbf{+0} & \textbf{0.79} & \textbf{0.64} \\
  ran14x18-disj-8 &\textbf{3} & 1.52k & 446.14k & \textbf{+0} & \textbf{0.67} & \textbf{0.55} & \textbf{+0} & 0.78 & 0.64 \\
  rd-rplusc-21 &0 & - & - & \textbf{+1} & - & - & +0 & - & - \\
  reblock115 &1 & 5.77k & \textbf{802.39k} & \textbf{+1} & \textbf{0.87} & 1.04 & +0 & 1.07 & 1.07 \\
  rmatr100-p10 &\textbf{3} & 174.13 & 857.67 & \textbf{+0} & 1.04 & 1.11 & \textbf{+0} & \textbf{1.00} & \textbf{0.97} \\
  rocI-4-11 &\textbf{3} & \textbf{727.85} & \textbf{13.22k} & -1 & 5.34 & 8.54 & \textbf{+0} & 2.51 & 2.56 \\
  rococoC10-001000 &\textbf{3} & 985.13 & 74.65k & \textbf{+0} & 0.89 & 1.30 & \textbf{+0} & \textbf{0.52} & \textbf{0.53} \\
  roi2alpha3n4 &\textbf{3} & \textbf{844.00} & \textbf{5.64k} & \textbf{+0} & 1.51 & 1.97 & \textbf{+0} & 1.21 & 1.30 \\
  roll3000 &\textbf{3} & 46.90 & 2.59k & \textbf{+0} & \textbf{0.75} & \textbf{0.61} & \textbf{+0} & 1.05 & 1.02 \\
  s250r10 &2 & 3.00k & 28.38k & \textbf{+1} & 1.41 & 1.58 & \textbf{+1} & \textbf{0.92} & \textbf{0.45} \\
  seymour1 &\textbf{3} & 60.80 & 1.49k & \textbf{+0} & \textbf{0.91} & \textbf{0.74} & \textbf{+0} & 1.00 & 0.77 \\
  sp98ar &0 & - & - & +0 & - & - & \textbf{+1} & - & - \\
  supportcase18 &\textbf{1} & - & - & -1 & - & - & -1 & - & - \\
  supportcase26 &1 & 6.16k & 7.60m & \textbf{+2} & \textbf{0.20} & \textbf{0.22} & +1 & 0.28 & 0.30 \\
  supportcase33 &\textbf{3} & 1.67k & 15.08k & \textbf{+0} & 1.23 & 1.20 & \textbf{+0} & \textbf{0.82} & \textbf{0.69} \\
  supportcase40 &\textbf{3} & 1.11k & 12.08k & \textbf{+0} & 1.05 & 1.05 & \textbf{+0} & \textbf{0.98} & \textbf{0.97} \\
  supportcase7 &\textbf{3} & 177.13 & \textbf{28.33} & \textbf{+0} & \textbf{1.00} & 1.05 & \textbf{+0} & 1.00 & 1.06 \\
  swath1 &\textbf{3} & 14.93 & 387.00 & \textbf{+0} & 1.03 & 1.05 & \textbf{+0} & \textbf{0.99} & \textbf{0.94} \\
  swath3 &\textbf{3} & 425.53 & 72.00k & \textbf{+0} & \textbf{0.33} & 0.32 & \textbf{+0} & 0.38 & \textbf{0.30} \\
  tbfp-network &\textbf{3} & \textbf{1.02k} & \textbf{51.00} & -1 & 3.36 & 6.81 & \textbf{+0} & 1.84 & 3.28 \\
  timtab1 &\textbf{3} & \textbf{52.40} & \textbf{39.40k} & \textbf{+0} & 1.22 & 1.33 & \textbf{+0} & 1.25 & 1.33 \\
  tr12-30 &\textbf{3} & 832.57 & 501.01k & \textbf{+0} & \textbf{0.73} & \textbf{0.72} & \textbf{+0} & 1.04 & 1.00 \\
  uct-subprob &\textbf{3} & 2.50k & 94.91k & \textbf{+0} & 0.78 & 0.81 & \textbf{+0} & \textbf{0.76} & \textbf{0.73} \\
  unitcal\_7 &\textbf{3} & \textbf{280.30} & 180.33 & \textbf{+0} & 1.02 & 0.96 & \textbf{+0} & 1.00 & \textbf{0.60} \\
  var-smallemery-m6j6 &0 & - & - & +0 & - & - & \textbf{+1} & - & - \\
  wachplan &\textbf{3} & \textbf{857.33} & \textbf{45.68k} & \textbf{+0} & 1.14 & 1.16 & \textbf{+0} & 1.13 & 1.10 \\

==> rubberband_large.tex <==
assign1-5-8 &\textbf{3} & 3.35k & 5.94m & \textbf{+0} & 0.96 & 0.93 & \textbf{+0} & \textbf{0.85} & \textbf{0.83} \\
bppc4-08 &0 & - & - & \textbf{+2} & - & - & \textbf{+2} & - & - \\
cost266-UUE &\textbf{3} & 3.18k & 234.69k & \textbf{+0} & 1.34 & 1.46 & \textbf{+0} & \textbf{0.96} & \textbf{0.95} \\
csched007 &\textbf{3} & 3.11k & 266.24k & \textbf{+0} & \textbf{0.53} & \textbf{0.51} & \textbf{+0} & 0.71 & 0.57 \\
csched008 &\textbf{3} & \textbf{1.03k} & \textbf{94.19k} & \textbf{+0} & 1.27 & 1.24 & \textbf{+0} & 1.36 & 1.42 \\
drayage-25-23 &\textbf{3} & 1.29k & \textbf{106.45k} & -2 & 4.99 & 18.14 & -2 & \textbf{0.97} & 2.67 \\
fastxgemm-n2r6s0t2 &\textbf{3} & 605.93 & 113.70k & \textbf{+0} & 1.35 & 1.42 & \textbf{+0} & \textbf{0.76} & \textbf{0.73} \\
gen-ip002 &\textbf{3} & 1.55k & 5.59m & \textbf{+0} & \textbf{0.91} & \textbf{0.93} & \textbf{+0} & 0.96 & 1.00 \\
gen-ip054 &\textbf{3} & 3.04k & 12.77m & \textbf{+0} & \textbf{0.63} & \textbf{0.62} & \textbf{+0} & 0.63 & 0.63 \\
glass-sc &\textbf{3} & 3.16k & 278.80k & \textbf{+0} & \textbf{0.93} & \textbf{0.96} & \textbf{+0} & 0.95 & 0.98 \\
glass4 &\textbf{3} & \textbf{2.17k} & \textbf{1.73m} & \textbf{+0} & 1.54 & 2.37 & \textbf{+0} & 1.14 & 1.63 \\
graph20-20-1rand &2 & 5.17k & 38.68k & +0 & \textbf{0.34} & \textbf{0.37} & \textbf{+1} & 0.49 & 0.49 \\
graphdraw-domain &\textbf{3} & \textbf{1.39k} & \textbf{2.52m} & \textbf{+0} & 1.15 & 1.11 & \textbf{+0} & 1.03 & 1.01 \\
icir97\_tension &0 & - & - & \textbf{+3} & - & - & +1 & - & - \\
markshare\_4\_0 &\textbf{3} & 320.37 & 2.51m & \textbf{+0} & \textbf{0.78} & \textbf{0.79} & \textbf{+0} & 0.87 & 0.88 \\
mas74 &\textbf{3} & 2.29k & 7.07m & \textbf{+0} & 0.89 & 0.84 & \textbf{+0} & \textbf{0.77} & \textbf{0.78} \\
mas76 &\textbf{3} & 132.87 & 301.16k & \textbf{+0} & 0.98 & 1.02 & \textbf{+0} & \textbf{0.90} & \textbf{0.88} \\
neos-1456979 &\textbf{1} & - & - & -1 & - & - & -1 & - & - \\
neos-2657525-crna &0 & - & - & +0 & - & - & \textbf{+1} & - & - \\
neos-3024952-loue &2 & 1.22k & 135.87k & \textbf{+1} & 1.25 & 0.92 & \textbf{+1} & \textbf{0.99} & \textbf{0.74} \\
neos-3627168-kasai &0 & - & - & \textbf{+1} & - & - & \textbf{+1} & - & - \\
neos-4738912-atrato &\textbf{3} & 1.02k & 103.05k & \textbf{+0} & \textbf{0.71} & \textbf{0.60} & \textbf{+0} & 0.87 & 0.82 \\
neos-5107597-kakapo &\textbf{3} & \textbf{2.10k} & \textbf{682.60k} & -2 & 2.67 & 3.52 & -1 & 1.85 & 2.23 \\
neos-911970 &\textbf{2} & \textbf{1.12k} & \textbf{623.61k} & -1 & 2.55 & 2.37 & -1 & 2.32 & 1.27 \\
neos5 &\textbf{3} & 104.37 & 255.57k & \textbf{+0} & \textbf{0.92} & \textbf{0.96} & \textbf{+0} & 1.12 & 1.19 \\
pg5\_34 &\textbf{3} & 2.09k & 191.13k & \textbf{+0} & 0.84 & 0.98 & \textbf{+0} & \textbf{0.72} & \textbf{0.90} \\
pk1 &\textbf{3} & 149.93 & 386.87k & \textbf{+0} & 1.03 & 1.06 & \textbf{+0} & \textbf{0.96} & \textbf{0.96} \\
ran14x18-disj-8 &\textbf{3} & 1.52k & 446.14k & \textbf{+0} & \textbf{0.67} & \textbf{0.55} & \textbf{+0} & 0.78 & 0.64 \\
rd-rplusc-21 &0 & - & - & \textbf{+1} & - & - & +0 & - & - \\
reblock115 &1 & 5.77k & \textbf{802.39k} & \textbf{+1} & \textbf{0.87} & 1.04 & +0 & 1.07 & 1.07 \\
rocI-4-11 &\textbf{3} & \textbf{727.85} & \textbf{13.22k} & -1 & 5.34 & 8.54 & \textbf{+0} & 2.51 & 2.56 \\
rococoC10-001000 &\textbf{3} & 985.13 & 74.65k & \textbf{+0} & 0.89 & 1.30 & \textbf{+0} & \textbf{0.52} & \textbf{0.53} \\
s250r10 &2 & 3.00k & 28.38k & \textbf{+1} & 1.41 & 1.58 & \textbf{+1} & \textbf{0.92} & \textbf{0.45} \\
sp98ar &0 & - & - & +0 & - & - & \textbf{+1} & - & - \\
supportcase18 &\textbf{1} & - & - & -1 & - & - & -1 & - & - \\
supportcase26 &1 & 6.16k & 7.60m & \textbf{+2} & \textbf{0.20} & \textbf{0.22} & +1 & 0.28 & 0.30 \\
swath3 &\textbf{3} & 425.53 & 72.00k & \textbf{+0} & \textbf{0.33} & 0.32 & \textbf{+0} & 0.38 & \textbf{0.30} \\
timtab1 &\textbf{3} & \textbf{52.40} & \textbf{39.40k} & \textbf{+0} & 1.22 & 1.33 & \textbf{+0} & 1.25 & 1.33 \\
tr12-30 &\textbf{3} & 832.57 & 501.01k & \textbf{+0} & \textbf{0.73} & \textbf{0.72} & \textbf{+0} & 1.04 & 1.00 \\
uct-subprob &\textbf{3} & 2.50k & 94.91k & \textbf{+0} & 0.78 & 0.81 & \textbf{+0} & \textbf{0.76} & \textbf{0.73} \\
var-smallemery-m6j6 &0 & - & - & +0 & - & - & \textbf{+1} & - & - \\
wachplan &\textbf{3} & \textbf{857.33} & \textbf{45.68k} & \textbf{+0} & 1.14 & 1.16 & \textbf{+0} & 1.13 & 1.10 \\
\midrule
Total & 93 & 144.30k & 134.87m & +4 & 1.00 & 0.87 & \textbf{+5} & \textbf{0.86} & \textbf{0.81} \\
Geo. mean & & 1.02k & 326.96k &  & 0.96 & 1.02 &  & \textbf{0.89} & \textbf{0.89} \\
Sh. geo. mean & &1.03k & 327.19k &  & 0.96 & 1.02 &  & \textbf{0.89} & \textbf{0.89} \\
